On modeling for Kerr black holes: Basis learning, QNM frequencies, and spherical-spheroidal mixing coefficients

Models of black hole properties play an important role in the ongoing direct detection of gravitational waves from black hole binaries. One important aspect of model based gravitational wave detection, and subsequent estimation of source parameters, are the low level modeling of information related to perturbed Kerr black holes. Here, we present new phenomenological methods to model the analytically understood gravitational wave spectra (quasi-normal mode frequencies), and harmonic structure of Kerr black holes (mixing coefficients between spherical and spheroidal harmonics). In particular, we present a greedy-multivariate-polynomial (GMVP) regression method and greedy-multivariate-rational (GMVR) regression method for the automated modeling of polynomial and rational functions respectively. GMVR is a quasi-linear numerical method for interpolating rational functions. It therefore represents a solution to Runge's phenomenon. GMVP is used to develop a model for QNM frequencies that explicitly enforces consistency with the extremal Kerr limit. GMVR is used to develop a model for harmonic mixing coefficients that extends previous results to dominant multipoles with $\ell \le 5$. Both models are the first of their kind to consider black hole spin to vary between -1 and 1, thus naturally connecting the pro and retrograde modes. We discuss the potential use of these models in current and future gravitational wave signal modeling.

==> fit_eqns.tex <==
% QNM fitting functions. This file was created by bhspec_latex_fit_eqns_fun.m
\begin{align}
	\label{eq:fit_fun_A220}
	A_{220}(\eta) \; &= \; \omega_{220}^2  \, (\, 0.9585 \, e^{ 2.9932 i} \eta + 0.4759 \, e^{ 0.8266 i} \eta^{2} + 1.2385 \, e^{ 2.3053 i} \eta^{3} \, )\\ 
	\label{eq:fit_fun_A221}
	A_{221}(\eta) \; &= \; \omega_{221}^2  \, (\, 0.1275 \, e^{ 0.0581 i} \eta + 1.1882 \, e^{ 1.5180 i} \eta^{2} + 8.2709 \, e^{ 4.4201 i} \eta^{3} + 26.2329 \, e^{ 1.1678 i} \eta^{4} \, )\\ 
	\label{eq:fit_fun_A210}
	A_{210}(\eta) \; &= \; \omega_{210}^2 \, \sqrt{1-4\eta} \, (\, 0.4795 \, e^{ 5.9656 i} \eta + 1.1736 \, e^{ 3.9747 i} \eta^{2} + 1.2303 \, e^{ 2.1732 i} \eta^{3} \, )\\ 
	\label{eq:fit_fun_A330}
	A_{330}(\eta) \; &= \; \omega_{330}^2 \, \sqrt{1-4\eta} \, (\, 0.4247 \, e^{ 4.5473 i} \eta + 1.4742 \, e^{ 2.7019 i} \eta^{2} + 4.3139 \, e^{ 5.1282 i} \eta^{3} + 15.7264 \, e^{ 2.2547 i} \eta^{4} \, )\\ 
	\label{eq:fit_fun_A331}
	A_{331}(\eta) \; &= \; \omega_{331}^2 \, \sqrt{1-4\eta} \, (\, 0.1480 \, e^{ 2.0396 i} \eta + 1.4874 \, e^{ 5.8954 i} \eta^{2} + 10.1637 \, e^{ 3.2835 i} \eta^{3} + 29.4786 \, e^{ 0.8106 i} \eta^{4} \, )\\ 
	\label{eq:fit_fun_A320}
	A_{320}(\eta) \; &= \; \omega_{320}^2  \, (\, 0.1957 \, e^{ 0.5433 i} \eta + 1.5830 \, e^{ 4.2451 i} \eta^{2} + 5.0338 \, e^{ 1.7100 i} \eta^{3} + 3.7366 \, e^{ 5.1474 i} \eta^{4} \, )\\ 
	\label{eq:fit_fun_A440}
	A_{440}(\eta) \; &= \; \omega_{440}^2  \, (\, 0.2531 \, e^{ 5.1632 i} \eta + 2.4040 \, e^{ 2.4690 i} \eta^{2} + 14.7273 \, e^{ 5.5624 i} \eta^{3} + 67.3624 \, e^{ 2.1982 i} \eta^{4} + 126.5858 \, e^{ 5.4174 i} \eta^{5} \, )\\ 
	\label{eq:fit_fun_A430}
	A_{430}(\eta) \; &= \; \omega_{430}^2 \, \sqrt{1-4\eta} \, (\, 0.0938 \, e^{ 2.3077 i} \eta + 0.8273 \, e^{ 6.1005 i} \eta^{2} + 3.3385 \, e^{ 3.8733 i} \eta^{3} + 4.6639 \, e^{ 1.7517 i} \eta^{4} \, )\\ 
	\label{eq:fit_fun_A550}
	A_{550}(\eta) \; &= \; \omega_{550}^2 \, \sqrt{1-4\eta} \, (\, 0.1548 \, e^{ 1.0675 i} \eta + 1.5091 \, e^{ 4.5498 i} \eta^{2} + 8.9333 \, e^{ 1.2898 i} \eta^{3} + 42.3431 \, e^{ 4.1004 i} \eta^{4} + 89.1947 \, e^{ 1.0251 i} \eta^{5} \, )
\end{align}

